Fourier Theory on the Complex Plane I: Conjugate Pairs of Fourier Series and Inner Analytic Functions

A correspondence between arbitrary Fourier series and certain analytic functions on the unit disk of the complex plane is established. The expression of the Fourier coefficients is derived from the structure of complex analysis. The orthogonality and completeness relations of the Fourier basis are derived in the same way. It is shown that the limiting function of any Fourier series is also the limit to the unit circle of an analytic function in the open unit disk. An alternative way to recover the original real functions from the Fourier coefficients, which works even when the Fourier series are divergent, is thus presented. The convergence issues are discussed up to a certain point. Other possible uses of the correspondence established are pointed out.

==> packages.tex <==
% JLdL 17Apr14.
%
% These are the packages to be used for the
% _ Mathematical Physics I/II lectures.
\usepackage[brazil]{babel}
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{epsfig}
\usepackage{amsfonts}
\usepackage{color}
\definecolor{lgrey}{gray}{0.99}

